Lang-n-Send: Processes That Send Languages

We present Lang-n-Send, a pi-calculus that is equipped with language definitions. Processes can define languages in operational semantics, and use them to execute programs. Furthermore, processes can send and receive pieces of operational semantics through channels. We present a reduction semantics for Lang-n-Send, and we offer examples that demonstrate some of the scenarios that Lang-n-Send captures.

==> eptcsdata.tex <==
\providecommand{\firstpage}{46}
\providecommand{\publicationstatus}{M. Carbone and R. Neykova (Eds.): 13th International\\
Workshop on Programming Language Approaches to\\
Concurrency and Communication-cEntric Software\\
EPTCS 356, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.356.5}{10.4204/EPTCS.356.5}}

